Sur la cohomologie \`a support des fibr\'es en droites sur les vari\'et\'es sym\'etriques compl\`etes

Let $X$ be a complete symmetric variety i.e. the wonderful compactification of a symmetric $G-$homogeneous space (where $G$ is a simply-connected semi-simple linear algebraic group). If $L$ is a line bundle over $X$ and if $C$ is a Bialynicki-Birula cell of codimension $c$ in $X$, then the Lie algebra $\mathfrak g$ of $G$ operates naturally on the cohomology group with support : $H^c_C(L)$. One gives here a necessary condition on the cell $C$ for that $\mathfrak g-$module have a finite dimensional simple subquotient. As applications one calculates the Euler-Poincar\'e characteristic of $L$ over $X$ and one estimates the higher cohomology group $H^d(X,L)$, $d \ge 0$, with exact formulae in some cases among which the case of the complete conic variety. -- \'Etant donn\'e un groupe alg\'ebrique lin\'eaire semi-simple G, on s'int\'eresse aux compactifications magnifiques des G?espaces homog\`enes sym\'etriques. Si X est une telle compactification, si L est un fibr\'e en droites G?lin\'earis\'e sur X et si C est une cellule de Bialynicki-Birula de X de codimension c, alors l'alg\`ebre de Lie g de G op\`ere naturellement sur le groupe de cohomologie \`a support Hc C (L). On donne ici une condition n\'ecessaire, portant sur la cellule C, pour que ce g?module poss\`ede un sous-quotient simple de dimension finie. On en d\'eduit une formule pour la caract\'eristique d'Euler-Poincar\'e de L sur X et une estimation (exacte pour certains cas dont celui de la vari\'et\'e des coniques compl\`etes) des groupes de cohomologie sup\'erieure Hd(X,L), d ? 0.

==> resume.tex <==
 \'Etant donn\'e un groupe alg\'ebrique lin\'eaire semi-simple $G$, on s'int\'eresse aux compactifications magnifiques des $G-$espaces homogènes sym\'etriques. Si $X$ est une telle compactification, si $L$ est un fibr\'e en droites $G-$lin\'earis\'e sur $X$ et si $C$ est une cellule de Bialynicki-Birula de $X$ de codimension $c$, alors l'algèbre  de Lie $\goth g$ de $G$ opère naturellement sur le groupe de cohomologie \`a support $H^c_C(L)$. On donne ici une condition n\'ecessaire, portant sur la cellule $C$, pour que ce $\goth g-$module possède un sous-quotient simple de dimension finie. On en d\'eduit une formule pour la caract\'eristique d'Euler-Poincar\'e de $L$ sur $X$ et une estimation (exacte pour certains cas dont celui de la vari\'et\'e des coniques complètes) des groupes de cohomologie sup\'erieure $H^d(X,L)$, $d \ge 0$.




==> titre.tex <==
Sur la cohomologie \`a support des fibr\'es en droites sur les vari\'et\'es sym\'etriques compl\`etes

